Ice Hockey Puck Localization Using Contextual Cues

Puck detection in ice hockey broadcast videos poses significant challenges due to the puck's small size, frequent occlusions, motion blur, broadcast artifacts, and scale inconsistencies due to varying camera zoom and broadcast camera viewpoints. Prior works focus on appearance-based or motion-based cues of the puck without explicitly modelling the cues derived from player behaviour. Players consistently turn their bodies and direct their gaze toward the puck. Motivated by this strong contextual cue, we propose Puck Localization Using Contextual Cues (PLUCC), a novel approach for scale-aware and context-driven single-frame puck detections. PLUCC consists of three components: (a) a contextual encoder, which utilizes player orientations and positioning as helpful priors; (b) a feature pyramid encoder, which extracts multiscale features from the dual encoders; and (c) a gating decoder that combines latent features with a channel gating mechanism. For evaluation, in addition to standard average precision, we propose Rink Space Localization Error (RSLE), a scale-invariant homography-based metric for removing perspective bias from rink space evaluation. The experimental results of PLUCC on the PuckDataset dataset demonstrated state-of-the-art detection performance, surpassing previous baseline methods by an average precision improvement of 12.2% and RSLE average precision of 25%. Our research demonstrates the critical role of contextual understanding in improving puck detection performance, with broad implications for automated sports analysis.

==> sec/intro_1.tex <==
\section{Introduction}

Computer vision has been widely used for ice hockey analytics \cite{}. The applications have expanded from player detection/ tracking \cite{}, pose estimation \cite{}, and jersey number recognition \cite{}. Recently, more advanced tasks, including shot prediction \cite{}, gameplay strategy analysis \cite{}, and puck possession estimation \cite{}, are also been studied. However, a common underlying factor in most of these tasks is the understanding of the precise prediction location of the puck, which provides crucial insight into game dynamics.

Given its fundamental importance in ice hockey analytics, accurate puck detection from broadcast video is essential~\cite{trackingimportant}, developing systems that assist coaches~\cite{}, and a general understanding of the ice hockey game. Although ball detection and tracking has been extensively studied in different sports such as soccer~\cite{4607578, Beetz2009ASPOGAMOAS, probtracksoccer, tvtracksoceer, leo_marco, REN2009633,VicenteMartnez2023AdaptationOY, balltracksoccer}, volleyball~\cite{4217275, volleyballtrajectory, chengvolley, chengnumber2}, and basketball~\cite{chakbasket, Chakraborty2012RealtimePE, chakdontmiss}, there is limited research on puck tracking in ice hockey games~\cite{vats2021puck, li2023ice, sarkhoosh_ai-based_2024, FollowThatPuck2017, pidaparthy2019keep}. 

Puck localization in broadcast videos is uniquely challenging due to occlusions, motion blur, in-the-air pucks, broadcast view artifacts (e.g., player nametag overlays, similarly shaped objects), the puck's tiny size, yellow-line pucks, and goal-line pucks. Occlusions from hockey player sticks, rink boards, and player bodies that obstruct the camera view of the puck significantly limit the performance of puck tracking. The high-speed motion of the puck causes motion blur and shape deformation due to its small size- just 0.005\% of the frame's pixel count \cite{yang2021puck}. 

Prior works tackle these issues by proposing various methods. XXXXXXXX. However, these methods rely heavily on manual thresholding or multiple contextual information (flow maps, player detection mask, etc.) with shallow networks. \textit{We argue that the fundamental issue in ice hockey puck detection is visual perspective distortion due to zooming of the broadcast camera, viewpoint variations, and setup of the broadcast camera in the rink.}

To tackle this challenge, we propose Position-Oriented Understanding for Contextual Constraint Keypoint Detection (PUCCKD), a context-aware multi-scale puck detection technique. Our approach integrates a context encoder to extract player masks, providing an \textit{implicit player position prior}. Then, a feature pyramid encoder with gated decoding embeds multi-scale feature information to \textit{tackle this scale issue}. The output heatmap from the gated decoder is then regressed to predict the puck's center position. In addition, we propose a new metric for unbiased evaluation without perspective distortion. Our main contributions can be summarized as follows:

\begin{itemize}
    \item We propose Position-Oriented Understanding for Contextual Constraint Keypoint Detection (PUCCKD), a contextually constrained feature pyramid network that adapts gated feature fusion at multiple scales, reducing false positive rates in detections.
    \item We introduce Rink-Space Localization Error (RSLE), an unbiased evaluation metric for puck detection that leverages homography-based detection error computation on ice hockey rink templates.
    \item Experimentation with VIP-PuckDataset shows state-of-the-art performance over baseline models, achieving a XX\% and \textbf{12.2\%} improvement in RSLE nad average precision.
\end{itemize}

==> sec/method_1.tex <==
\subsection{Model Architecture} % NEEDS A REWRITE !!!
\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{fig/inference.png}
    \caption{Left image (within blue dots) includes context image generation pipeline, a combination of detection and segmentation models frozen in training. The right image (within red dots) is the trained PUCCKD model architecture.}
    \label{fig:model_arch}
\end{figure*}

\section{Methodology}

\subsection{Overview}

Our PUCCKD architecture consists of two parts: 1) \textbf{Context Encoder}, which extracts player segmentation masks to provide spatial context from the input image; and 2) $<Main Architecture>$, which utilizes a feature pyramid encoder with gated decoding to predict robust heatmap representations for puck localization. These heatmap representations are then regressed to predict the puck's center position. Figure \ref{fig:model_arch} shows the network architecture of PUCCKD used to regress the puck positions. 

\subsection{$<Main Architecture>$} %to be named..

% FORMULATE THE PROBLEM HERE
Given the input image $\mathcal{I}$, the Context Encoder (CE) extracts a corresponding segmentation mask $\mathcal{M}$ from input $\mathcal{I}$. Then, the Feature Pyramid Encoder (FPE) predicts multiscale representations $Z_I$ and $Z_M$ from the image and mask, respectively. These representations are then fed as input to the gated decoder $\mathcal{D}$, which combines them to generate the heatmap representation $Y$. Finally, the heatmap ($Y$) is regressed to predict the puck centers ($\hat{Y}$). 

\subsection{Context Encoder} %it would be better to rename this with an understanding of what the context is- "players". it does make sense to name it context if we don't know the context explicitly, but here we do. Think about this!

% Also, I don't think having context image and context encoder in 2 different places helps the reviewers/readers. 

% Avoid referring to topics like "gated decoder" in this section when it is not explained yet. And in methodology, u don't have to compare and contrast ur mechanism with other plausible approaches. 

% ur original content under this topic had some explanation looping in FPNs. I would rather just talk abt the motivation behind context encoding and finish this subsection. And then loop it in for the main architecture. I would suggest something like this:

For the task of puck detection, relying solely on the visual puck information is impractical due to the small size of the puck and the dynamic nature of the game, which often involves significant occlusion and motion blur. Therefore, incorporating additional context is crucial to guide the models toward robust puck localization. 

Prior research has revealed a significant correlation between the puck location and the pose of the players in the rink \cite{}. However, directly extracting player pose, as explored in \cite{}, is computationally expensive, and the pose estimator struggles with occlusion and motion blur issues.

Considering these factors, we propose using a simple segmentation mask of each player as a valid contextual input. To do so, we first extract the bounding box of each player using a pretrained detector \cite{yolo} and then segment the detected players using a pretrained segmentation algorithm \cite{sam2}. The resulting output is then processed into a binary mask to provide contextual information to the localization task. 

% JUST RE-READ UR RESOLUTION PARA (h/2, w/2). Would changing just the h and w not affect the fusion process since both will be in different scales? I don't quite understand that part. It would be easier I think if u could explain all this in the pyramid encoder so that everything in regards to the scale will be under one roof!

\paragraph{Feature Pyramid Encoder}

In sports analytics, the broadcast camera angle and its zoom level significantly influence the perceived object's scale within the image. Thus, a multiscale understanding of features between images is crucial for accurate and adaptable localization \cite{}. Prior works relied on methods that operate on a single scale and XXXX \cite{}. 

To that end, we propose FPE, which inputs the image ($\mathcal{I}$) and the segmentation mask ($\mathcal{M}$) as input to predict the heatmap representation ($Y$). TALK ABT THE PYRAMID CONSTRUCTION! 

\paragraph{Gated Decoder}

To effectively fuse the multiscale features $Z_I$ and $Z_M$ to localize the puck, we utilize a gated decoder. At the decoding stage, $Z_I$ and $Z_M$ are concatenated through the decoder ($\mathcal{D}$) that learns per-channel weights via a sigmoid function. This can be formulated as:

\begin{equation}
    Z' = \mathcal{D}(Z_I, Z_M) = \lambda_I Z_I + \lambda_M Z_M
\end{equation}

% Let's not talk abt inference weighing here. That has to be in experimentation as well. 

\noindent where, $\lambda_I$ and $\lambda_M$ are the learnable weights of the decoder ($\mathcal{D}$) with the output features denoted with $Z'$. This static gating is reminiscent of Squeeze-and-Excitation blocks, which derive channel re-weightings based on global channel context \cite{squeeze}.

% Saw ur comments for the dual strategy with Amir. We can argue since u have the results. But that para should be in the experimentation following the table, not here!

\paragraph{Heatmap Representation.} CHECK THE PAGE COMMENTS!!
% Talk abt how u go from decoded features ($Z'$) to $Y$ and then to $\hat{Y}$ via regression here. Basically the MLP block u used. 

% If loss is estimated using the heatmap and not the puck center, then don't talk abt regressing here to get $\hat{Y}$ here. 

\subsection{Objective Function}

The PUCCKD model is trained to minimize the distance between the predicted and groundtruth puck centers. To do so, we utilize Kullback-Leibler divergence loss ($\mathcal{L}_{KL}$) to penalize spatial displacement, encouraging the network to predict a peak precisely at the correct point. 

% The input for the loss fn is not clear- What are the inputs- heatmap gt and pred or puck center gt and pred? Were any LOG operations done here? An eqn would help the readers. 

% I removed ur explanation of why it is better than MSE here because it makes more sense to have it in the ablation study. I am assuming u have a model trained with MSE as well.  

\section{RSLE Evaluation Metric}

% \noindent \textbf{NEED FOR A NEW METRIC?}
Conventional metrics like average precision/ pixel-space distance measures have inherent limitations due to the camera's perspective distortion. That is, these metrics are highly influenced by the different camera zooms, viewpoints, and broadcast setups, resulting in skewed model evaluation.   

To address these issues, we propose Rink-Space Localization Error 
(\textit{RSLE}), a novel evaluation metric to measure the puck detection accuracy in a transformed rink coordinate system. The RSLE metric can be formulated as:

\begin{equation}
    D_{rink} = \sqrt{(\hat{x}_{rink} - x_{rink})^2 + (\hat{y}_{rink} - y_{rink})^2}
\end{equation}

\noindent where, $\hat{x}_{rink}$ and $\hat{y}_{rink}$ are the transformed puck coordinates in homography coordinates. Figure \ref{} shows the scale issue where the Euclidean distance is more by XX\%, while RSLE remains consistent in both cases by taking into account the scale. % I think adding an image to show a similar RSLE error but different euclidean or AP would be great!

\textbf{Homography Estimation.} To ensure accurate and consistent evaluation, we transform all the puck positions from image coordinates to homography coordinates. This transformation enables RSLE to be independent of the perspective distortion- camera viewpoint, lens distortion, or zoom level, thereby ensuring fairness. 

Homography establishes a projective transformation mapping the 2D image coordinates to a predefined rink-space representation. In this work, we utilize the homography technique proposed by Shang et al. \cite{homography}, which follows a three-stage process. First, the segmentation map of each input frame is extracted. Next, a coarse model aligns the segmentation map with the rink template ($\mathcal{R}$) to output the homography, providing an initial transformation estimate. Finally, a refinement stage adjusts the warped template to better match the orientation observed in the segmentation map. 

% LETS MOVE DATA PREPROCESSING SUBSECTION TO IMPLEMENTATION SUBSECTION OF EXPERIMENTATION. 
